Uncertainty-DTW for Time Series and Sequences

Dynamic Time Warping (DTW) is used for matching pairs of sequences and celebrated in applications such as forecasting the evolution of time series, clustering time series or even matching sequence pairs in few-shot action recognition. The transportation plan of DTW contains a set of paths; each path matches frames between two sequences under a varying degree of time warping, to account for varying temporal intra-class dynamics of actions. However, as DTW is the smallest distance among all paths, it may be affected by the feature uncertainty which varies across time steps/frames. Thus, in this paper, we propose to model the so-called aleatoric uncertainty of a differentiable (soft) version of DTW. To this end, we model the heteroscedastic aleatoric uncertainty of each path by the product of likelihoods from Normal distributions, each capturing variance of pair of frames. (The path distance is the sum of base distances between features of pairs of frames of the path.) The Maximum Likelihood Estimation (MLE) applied to a path yields two terms: (i) a sum of Euclidean distances weighted by the variance inverse, and (ii) a sum of log-variance regularization terms. Thus, our uncertainty-DTW is the smallest weighted path distance among all paths, and the regularization term (penalty for the high uncertainty) is the aggregate of log-variances along the path. The distance and the regularization term can be used in various objectives. We showcase forecasting the evolution of time series, estimating the Fr\'echet mean of time series, and supervised/unsupervised few-shot action recognition of the articulated human 3D body joints.

==> abstract.tex <==
\begin{abstract}


We model the so-called aleatoric uncertainty of a differentiable (soft) version of celebrated Dynamic Time Warping (DTW). The transportation plan of DTW contains a set of paths; each path matches frames between two sequences under a varying degree of time warping. However, the DTW distance, which is the smallest path-wise distance (the sum of base distances between features of pairs of frames of the path), is sub-optimal as it ignores the observation uncertainty which can vary per frame. Thus, we model the heteroscedastic aleatoric uncertainty of each path by the product of likelihoods from Normal distributions, each capturing a variance of pair of frames. The Maximum Likelihood Estimation (MLE) applied to each path yields a sum of variance-weighted Euclidean distances, and a sum of log-variance regularization terms. Then, our uncertainty-DTW distance is the smallest variance-weighted path-wise log-variances, and the regularization term (penalty for the high uncertainty) is the aggregate of path-wise log-variances. Both the distance and the regularization term can be used as components of various objective functions. We showcase forecasting the evolution of the time series, estimating the Fr\'echet mean of time series, and supervised and unsupervised few-shot action recognition of the articulated 3D human body joints.



% In this paper, we take a look at Soft-DTW, a differentiable version of Discrete Time Warping (DTW) for time series and action recognition. While its underlying transportation plan allows for some degree of warped match between a pair of sequences, inherently the most dominant matching path may be sub-optimal due to the underlying noise of frame-wise feature representations. For that reason, we drop the notion of the base distance of Soft-DTW. Specifically, we model each compared pair of sequences by the Normal distribution with a unique variance. Thus, each path of Soft-DTW is modeled as a product of likelihoods that can be maximized by the MLE. The log of likelihood results in a weighted Euclidean distance and a regularization term on the variance, which are both aggregated along the path. The smallest-distance path reflects the best matching distance given the set of variances along the path, whereas the corresponding accumulated regularization term penalizes for the high uncertainty (large variances). Both the distance and the regularization term can be used as components of the objective functions for various time series problems. We showcase applications such as forecasting the evolution of time series, estimating the Fr\'echet mean of time series, and supervised and unsupervised few-shot action recognition of the articulated 3D human body joints.
\keywords{time series, few-shot, acction recognition}
\end{abstract}

==> exper.tex <==
\section{Experiments}

Below we apply uDTW as a component of the objective functions for various time series problems including time series classification and action recognition tasks. 

\subsection{Datasets}

\noindent{{\em UCR}} archive~\cite{UCRArchive} is a dataset for time series classification archive. This dataset contains a wide variety of fields (astronomy, geology, medical imaging) and lengths, and can be used for time series classification/clustering and forecasting tasks.

\noindent{{\em NTU RGB+D (NTU-60)}}~\cite{Shahroudy_2016_NTURGBD} contains 56,880 video sequences and over 4 million frames. 
This dataset has variable sequence lengths  and exhibits high intra-class variations. %It is also known as NTU-60.

%\vspace{0.05cm}
\noindent{{\em NTU RGB+D 120 (NTU-120)}}~\cite{Liu_2019_NTURGBD120}, an extension of NTU-60, contains 120 action classes (daily/health-related), and 114,480 RGB+D video samples  captured with 106 distinct human subjects from 155 different camera viewpoints.

%\vspace{0.05cm}
\noindent{{\em Kinetics}}~\cite{kay2017kinetics} is a large-scale collection of 650,000 video clips that cover 400/600/700 human action classes.
It includes human-object interactions such as {\it playing instruments}, as well as human-human interactions such as {\it shaking hands} and {\it hugging}. 
% As the Kinetics-400 dataset provides only the raw videos, we follow approach~\cite{stgcn2018aaai} and use the estimated joint locations in the pixel coordinate system as the input to our pipeline. 
% To obtain the joint locations, we first resize all videos to the resolution of 340 $\times$ 256, and convert the frame rate to 30 FPS. Then we use the publicly available {\it OpenPose}~\cite{Cao_2017_CVPR} toolbox to estimate the location of 18 joints on every frame of the clips. 
We follow approach~\cite{stgcn2018aaai} and use the estimated joint locations in the pixel coordinate system as the input to our pipeline.
As OpenPose  produces the 2D body joint coordinates and Kinetics-400 does not offer multiview or depth data, we use a network of Martinez et al.   \cite{martinez_2d23d} pre-trained on Human3.6M~\cite{Catalin2014Human3}, combined with the 2D OpenPose output to  estimate 3D coordinates from 2D coordinates. The 2D OpenPose and the latter network give us $(x,y)$ and $z$ coordinates, respectively.

\subsection{Fr\'echet mean of time series}

In this section, we compare the uDTW barycenter approach to Euclidean and sDTW.


\begin{figure}[t]
\centering%%%%
%\vspace{-0.3cm}
%\vspace{0.1cm}
\begin{subfigure}[b]{0.40\linewidth}
\includegraphics[trim=1cm 1cm 1cm 2.5cm, clip=true,width=0.99\linewidth]{imgs/lambda1_uncertainty_with_euc_beta-10-1-0.1-sdtw-sdtw-unc.pdf}% \vspace{-0.2cm}
\caption{$\beta$}\label{fig:beta}
%\vspace{-0.2cm}
\end{subfigure}
%
\begin{subfigure}[b]{0.40\linewidth}
\includegraphics[trim=1cm 1cm 1cm 2.5cm, clip=true,width=0.99\linewidth]{imgs/beta1_uncertainty_with_euc_lambda-10-1-0.1-sdtw-sdtw-unc.pdf}% \vspace{-0.2cm}
\caption{$\lambda$}\label{fig:lambda}
%\vspace{-0.2cm}
\end{subfigure}
\caption{Interpolation between two time series (grey and black) on the Gun Point dataset. We compute the barycenter by solving Eq.~\ref{}.}
%\vspace{-0.3cm}
\label{fig:interp}
\end{figure}


\begin{figure*}[t]
\centering%%%%
%\vspace{-0.3cm}
%\vspace{0.1cm}
\begin{subfigure}[t]{0.7\linewidth}
\includegraphics[trim=14cm 1cm 1cm 1.2cm, clip=true,width=\linewidth]{imgs/CBF-udtw-barycenter-withsigmaNet.pdf}% \vspace{-0.2cm}
\caption{CBF}\label{fig:cbf}
%\vspace{-0.2cm}
\end{subfigure}\\
%
\begin{subfigure}[t]{0.7\linewidth}
\includegraphics[trim=14cm 1cm 1cm 1.2cm, clip=true,width=\linewidth]{imgs/ECG200-udtw-barycenter-withsigmaNet.pdf}% \vspace{-0.2cm}
\caption{ECG200}\label{fig:ecg200}
%\vspace{-0.2cm}
\end{subfigure}\\

\begin{subfigure}[t]{0.7\linewidth}
\includegraphics[trim=14cm 1cm 1cm 1.2cm, clip=true,width=\linewidth]{imgs/synthetic_control-udtw-barycenter-withsigmaNet.pdf}% \vspace{-0.2cm}
\caption{Synthetic Control}\label{fig:syn}
%\vspace{-0.2cm}
\end{subfigure}

\caption{Comparison of barycenter obtained by our uDTW and sDTW on CBF, ECG200 and Synthetic Control dataset. Left column $\gamma = 1$ and right column $\gamma = 10$ for both methods.}
%\vspace{-0.3cm}
\label{fig:barycenter}
\end{figure*}



\noindent{\bf Experimental setup.} For each dataset in UCR, we choose a class at random, pick 10 time series from this class and compute their barycenter. For each method, we set the maximum number of iterations to 100. We use L-BFGS to minimise the proposed uDTW barycenter objective.



\noindent{\bf Qualitative results.} We first do averaging interpolation between two time series (Figure~\ref{fig:interp}). We notice that averaging under the uDTW results in substantially different results than those that can be obtained with the Euclidean and sDTW geometry.

Figure~\ref{fig:barycenter} shows barycenters obtained using our uDTW and sDTW. We observe that our uDTW yields more reasonable barycenters than sDTW even when $\gamma=10$ (right column of plots in Figure~\ref{fig:barycenter}). We provide more visualizations in Appendix.



\subsection{Time series classification}

In this section, we validate the uncertainty in sDTW can act as a useful regularization and improve the classification accuracy. We choose two simple classifiers: nearest neighbor and nearest centroid~\cite{hastie01statisticallearning}. The nearest centroid classifier first computes the centroid (average) of each class in the training set. We compute the centroid by minimising the Fr\'echet mean for each class. To predict the class of a time series, we then assign the class of the nearest centroid. Although very simple, this method is known to be competitive with the nearest neighbour classifier, while requiring much lower computational cost at the prediction stage. 

% To predict the class of a time series, the well-known nearest neighbor classifier assigns the class of the nearest time series in the training set, according to the chosen method. 

\noindent{\bf Experimental setup.} We use 50\% of the data for training, 25\% for validation and 25\% for testing. We report $K=$ 1, 2 and 3 for the nearest neighbour.

\noindent{\bf Quantitative results.} Table~\ref{tab:ucrclassification} shows a comparison summary of our uDTW versus the use of Euclidean, DTW and sDTW. Unsurprisingly, the use of uDTW for barycenter computation improves the accuracy of the nearest centroid classifier, and the boosts for the use of nearest neighbour for $K$=1, 2 and 3 are 2.4\%, 1.3\% and 0.8\%, respectively.

% \begin{table}[t]
% \caption{Classification accuracy ((mean$\pm$std)) on UCR archive using nearest neighbor and nearest centroid classifiers.}
% \label{tab:ucrclassification}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lcccc}
% \toprule
%  & \multicolumn{3}{c}{\bf Nearest neighbour} &\!\!\!\!{\bf Nearest centroid}\!\!\!\\
%  \cline{2-4}
 
%  & $K = 1$ & $K = 3$ & $K = 5$ & \\
% \midrule
% \!\!\!Eucl. & \!\!\!71.2$\pm$17.5\!\!\!&\!\!\! 69.5$\pm$18.0\!\!\!& \!\!\!67.5$\pm$17.6\!\!\!\!\!&\!\!\!61.3$\pm$20.1\\
% \!\!\!DTW &\!\!\! 74.2$\pm$16.6\!\!\!&\!\!\!72.8$\pm$16.9\!\!\!&\!\!\!71.4$\pm$16.8\!\!\!\!\!&\!\!\!65.9$\pm$18.8 \\
% \!\!\!sDTW &\!\!\! 76.2$\pm$16.6\!\!\!&\!\!\!75.2$\pm$16.8\!\!\!&\!\!\! 74.0$\pm$15.6\!\!\!\!\!&\!\!\!70.5$\pm$17.6\\ 
% \!\!\!\!\!\!sDTW div\!\!\!&\!\!\! 78.6$\pm$16.2\!\!\!&\!\!\! 76.5$\pm$16.4\!\!\!&\!\!\!74.8$\pm$15.8\!\!\!\!\!&\!\!\! 70.9$\pm$17.8\\ 
% \hdashline
% 
% % \!\!\!uDTW\!\!\!\! &\!\!\! {\bf 78.6$\pm$16.2}\!\!\!&\!\!\!{\bf 76.5$\pm$16.4}\!\!\!&\!\!\!{\bf 74.8$\pm$15.8}\!\!\!\!\!&\!\!\!{\bf 70.9$\pm$17.8}\\
% \!\!\!uDTW\!\!\!\! &\!\!\! 80.0$\pm$15.0\!\!\!&\!\!\! 78.0$\pm$15.8\!\!\!&\!\!\!76.2$\pm$15.0\!\!\!\!\!&\!\!\! 72.2$\pm$16.0\\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}


\begin{table}[t]
\caption{Classification accuracy ((mean$\pm$std)) on UCR archive using nearest neighbor and nearest centroid classifiers.}
\label{tab:ucrclassification}
%\vskip 0.15in
\begin{center}
\begin{tabular}{lcccc}
\toprule
 & \multicolumn{3}{c}{\bf Nearest neighbour} &{\bf Nearest centroid}\\
 \cline{2-4}
 
 & $K = 1$ & $K = 3$ & $K = 5$ & \\
\midrule
Eucl. & 71.2$\pm$17.5& 72.3$\pm$18.1& 73.0$\pm$16.7&61.3$\pm$20.1\\
DTW~\cite{1163055} & 74.2$\pm$16.6&75.0$\pm$17.0&75.4$\pm$15.8&65.9$\pm$18.8 \\
sDTW~\cite{marco2017icml} & 76.2$\pm$16.6&77.2$\pm$15.9& 78.0$\pm$16.5&70.5$\pm$17.6\\ 
sDTW div~\cite{pmlr-v130-blondel21a}& 78.6$\pm$16.2& 79.5$\pm$16.7&80.1$\pm$16.5\!\!& 70.9$\pm$17.8\\ 
\hdashline

% uDTW\! & {\bf 78.6$\pm$16.2}&{\bf 76.5$\pm$16.4}&{\bf 74.8$\pm$15.8}\!\!&{\bf 70.9$\pm$17.8}\\
uDTW & 80.0$\pm$15.0& 81.2$\pm$17.8&83.3$\pm$16.2& 72.2$\pm$16.0\\
\bottomrule
\end{tabular}
\end{center}
\end{table}



\subsection{Forecasting experiments}
\noindent{\bf Experimental setup.} We use the training and test sets pre-defined in the UCR archive. For both training and test, we use the first 60\% of the time series as input and the remaining 40\% as output, ignoring the class information. In this experiments, we use a simple multi-layer perception (MLP) with one hidden layer and sigmoid function. For uDTW, we also have a small sigmaNet that consists of an FC layer and a sigmoid function to learn the uncertainty information.

\noindent{\bf Qualitative results.} The visualization of the predictions are given in Figure~\ref{fig:pred}. Although the predictions under the sDTW and uDTW losses sometimes agree with each other, they can be visibly different. Predictions under uDTW can confidently predict the abrupt and sharp changes.


\noindent{\bf Quantitative results.} We also provide quantitive results to validate the effectiveness of uDTW. We use ECG5000 dataset from the UCR archive which is composed of 5000 electrocardiograms (ECG) (500 got training and 4500 for testing) of length 140. To better evaluate the predictions, we use 3 metrics (i) MSE for the predicted errors (ii) sDTW, sDTW div and uDTW for the shape of time series. We then use the Student's $t$-test (with significance level 0.05) to highlight the best performance in each experiment (averaged over 100 runs). Table~\ref{tab:pred} summarises the results. 


\begin{figure}[t]
\centering%%%%
%\vspace{-0.3cm}
%\vspace{0.1cm}
\begin{subfigure}[b]{0.40\linewidth}
\includegraphics[trim=0.6cm 9.2cm 12.6cm 0cm, clip=true,width=0.99\linewidth]{imgs/ECG200_pred_.pdf}% \vspace{-0.2cm}
\caption{ECG200}\label{fig:ecg200_pred}
%\vspace{-0.2cm}
\end{subfigure}
%
\begin{subfigure}[b]{0.40\linewidth}
\includegraphics[trim=12.6cm 0.5cm 0.6cm 9cm, clip=true,width=0.99\linewidth]{imgs/ECG5000_pred_.pdf}% \vspace{-0.2cm}
\caption{ECG5000}\label{fig:ecg5000_pred}
%\vspace{-0.2cm}
\end{subfigure}
\caption{Given the first part of a time series and we train 3 multi-layer perception (MLP) to predict the entire second part. Using ECG200 and ECG5000 dataset, we use Euclidean, DTW, sDTW div and uDTW loss for each MLP. We display above the prediction obtained for the given test sample with either of these 3 MLPs in addition to the ground truth (GT). Oftentimes, we observe that the uDTW loss enables us to better predict the sharp changes.}
%\vspace{-0.3cm}
\label{fig:pred}
\end{figure}


\begin{table}[t]
\caption{Multistep-ahead prediction results evaluated with MSE, DTW, sDTW div and uDTW metrics on ECG5000, averaged over 100 runs (mean$\pm$std). 
% Metrics are scaled for readability ($\times$100 for MSE and the rest metrics are $\times$ 10) ). 
Best method(s) are highlighted in bold using Student's $t$-test.}
\label{tab:pred}
%\vskip 0.15in
\begin{center}

\begin{tabular}{lcccc}
\toprule
& Eucl. & sDTW & sDTW div & uDTW\\
\hline
MSE & {\bf 32.1$\pm$1.62}&38.6$\pm$6.30& 24.6$\pm$1.37& 23.0$\pm$1.22\\
DTW~\cite{1163055} &20.0$\pm$0.18&{\bf 17.2$\pm$0.80}&38.9$\pm$5.33&{\bf 16.7$\pm$0.08} \\
sDTW div~\cite{pmlr-v130-blondel21a} &15.3$\pm0.16$&22.6$\pm$3.59&{\bf 20.0$\pm$2.44}& {\bf 16.8$\pm$1.62}\\
uDTW &14.4$\pm$0.18&32.1$\pm$2.25& 15.4$\pm$1.62&{\bf 8.27$\pm$0.79} \\
\bottomrule
\end{tabular}
\end{center}
%\vskip -0.1in
\end{table}



\subsection{Supervised/unsupervised few-shot action recognition}

In this section, we use uDTW as a loss function for few-shot action recognition (AR) tasks. We conduct both supervised and unsupervised settings to validate the effectiveness of the proposed method. For both supervised and unsupervised, we use a 3-layer MLP unit with SSGC~\cite{hao2021iclr} followed by a transformer as backbone (refer to Appendix for network configuration and training details). For the unsupervised learning, we use Locality-constrained Soft Assignment (LCSA)~\cite{6126534,6116129} for the sparse coding and dictionary learning, and we use histogram intersection kernel to compare the generated sparse codes of each pair of the support and query samples. 

\noindent{\bf Experimental setup.} For NTU-120, we follow the standard one-shot protocols~\cite{Liu_2019_NTURGBD120}. Base on this protocol, we create a similar one-shot protocol for NTU-60, with 50/10 action classes used for training/testing respectively (see Appendix for the evaluation protocols). We also evaluate the model on both 2D and 3D Kinetics-skeleton. We split the whole dataset into 200 actions for training and the rest half for testing. 

\noindent{\bf Quantitative results.} Table~\ref{tab:ntu60},~\ref{tab:ntu120} and~\ref{tab:kinetics} shows the experimental results on few-shot action recognition. Our proposed uDTW performs better than sDTW on both supervised and unsupervised settings. On Kinetics-skeleton dataset, we gain 2.4\% and 4.4\% improvements on 3D skeletons for supervised and unsupervised respectively. More evaluation results on few-shot action recognition can be found in Appendix.


\begin{table}[tbp]

\begin{minipage}{.5\linewidth}

\caption{Evaluations on NTU-60. }
\label{tab:ntu60}
\centering
%\vskip 0.15in
% \begin{center}
\begin{tabular}{lccccc}
\toprule
\#classes & 10 & 20 & 30 & 40 & 50\\
\midrule
& \multicolumn{5}{c}{\bf Supervised}\\
\hline
MatchNets~\cite{f4Matching} 
& 46.1 & 48.6 & 53.3 & 56.3 & 58.8 \\
ProtoNet~\cite{f1} 
& 47.2 & 51.1 & 54.3 & 58.9 & 63.0 \\
TAP~\cite{su2022temporal}
& 54.2 & 57.3 & 61.7 & 64.7 & 68.3 \\
\hdashline
sDTW~\cite{marco2017icml} & 53.7 & 56.2 & 60.0 & 63.9 & 67.8\\
\rowcolor{blue!10}
% uDTW & {\bf 56.9} & {\bf 61.2} & {\bf 64.8} & {\bf 68.3} & {\bf 72.4}\\
uDTW & 56.9 & 61.2 & 64.8 & 68.3 & 72.4\\
\hline
& \multicolumn{5}{c}{\bf Unsupervised}\\
\hline
% & & & & & \\
% & & & & & \\
% \hdashline
sDTW~\cite{marco2017icml} & 35.6 & 45.2 & 53.3 & 56.7 & 61.7\\
\rowcolor{blue!10}
% uDTW & {\bf 37.0} & {\bf 48.3} & {\bf 55.3} & {\bf 58.0} & {\bf 63.3}\\
uDTW & 37.0 & 48.3 & 55.3 & 58.0 & 63.3\\
\bottomrule
\end{tabular}
\end{minipage}\hfill
\begin{minipage}{.5\linewidth}
\caption{Evaluations on NTU-120.}
\label{tab:ntu120}
\centering
%\vskip 0.15in
% \begin{center}
\begin{tabular}{lccccc}
\toprule
\#classes & 20 & 40 & 60 & 80 & 100\\
\midrule
& \multicolumn{5}{c}{\bf Supervised}\\
\hline
TAP~\cite{su2022temporal}
& 31.2 & 37.7 & 40.9 & 44.5 &  47.3\\
sDTW~\cite{marco2017icml} & 30.3 & 37.2 & 39.7 & 44.0 & 46.8\\
\rowcolor{blue!10}
% uDTW & {\bf 32.2} & {\bf 39.0} & {\bf 41.2} & {\bf 45.3} & {\bf 49.0}\\
uDTW & 32.2 & 39.0 & 41.2 & 45.3 & 49.0\\
\hline
& \multicolumn{5}{c}{\bf Unsupervised}\\
\hline
sDTW~\cite{marco2017icml} & 20.1 & 25.3 & 32.0 & 36.9 & 40.9\\
\rowcolor{blue!10}
% uDTW & {\bf 22.7} & {\bf 28.3} & {\bf 35.9} & {\bf 39.4} & {\bf 44.0}\\
uDTW & 22.7 & 28.3 & 35.9 & 39.4 & 44.0\\
\bottomrule
\end{tabular}
% \end{center}
%\vskip -0.1in
\end{minipage}
\end{table}


% \begin{table}[t]
% \caption{Evaluations on 2D and 3D Kinetics-skeleton.}
% \label{tab:kinetics}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lcc}
% \toprule
% &  2D skel. & 3D skel. \\
% \midrule
% & \multicolumn{2}{c}{\bf Supervised}\\
% \hline
% sDTW  & 34.7 & 39.6\\
% uDTW & 35.5 & {\bf 42.0}\\
% \hline
% & \multicolumn{2}{c}{\bf Unsupervised}\\
% \hline
% sDTW & 23.3 & 28.3\\
% uDTW & 25.9 & {\bf 32.7}\\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}

\begin{table}[t]
\caption{Evaluations on 2D and 3D Kinetics-skeleton.}
\label{tab:kinetics}
%\vskip 0.15in
\begin{center}
\begin{tabular}{lcccc}
\toprule
& \multicolumn{2}{c}{\bf Supervised} & \multicolumn{2}{c}{\bf Unsupervised}\\
\cline{2-5}
& 2D & 3D & 2D & 3D\\
\midrule
TAP~\cite{su2022temporal}
& 32.9 & 36.0 & - & -\\
sDTW~\cite{marco2017icml}  & 34.7 & 39.6 & 23.3& 28.3\\
\rowcolor{blue!10}
% uDTW & 35.5 & {\bf 42.0} & 25.9 & {\bf 32.7}\\
uDTW & 35.5 & 42.0 & 25.9 & 32.7\\
\bottomrule
\end{tabular}
\end{center}
%\vskip -0.1in
\end{table}
